The classification of dp-minimal integral domains

We classify dp-minimal integral domains, building off the existing classification of dp-minimal fields and dp-minimal valuation rings. We show that if R is a dp-minimal integral domain, then R is a field or a valuation ring or arises from the following construction: there is a dp-minimal valuation overring O extending R, a proper ideal I in O, and a finite subring S in O/I such that R is the preimage of S in O.

==> preamble.tex <==

%Margin
\usepackage{anysize}
\marginsize{3cm}{3cm}{3cm}{3cm}



\usepackage{amssymb,latexsym}
%\usepackage[utf8x]{inputenc} %/!\ this package is incompatible with biblatex
\usepackage{amsmath,amsthm}
\usepackage{amsfonts,mathrsfs}
\usepackage{mathtools}


%Times New Roman (choose one of the three):
%\usepackage{mathptmx} %<- choosen for MSCA
%\usepackage{newtxtext,newtxmath}
%\usepackage{times}

\usepackage{tikz-cd}

\usepackage{todonotes}

% \usepackage{enumerate,units}
\usepackage[all]{xy}
\usepackage{graphicx}

\usepackage{xcolor,url}
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    citecolor=blue,
    filecolor=blue,
    linkcolor=black,
    urlcolor=blue
}

%Times New Roman (choose one of the three):
%\usepackage{mathptmx} %<- choosen for MSCA


\usepackage[shortlabels]{enumitem}


% Headers and footers
% \usepackage{fancyhdr,lastpage}
% \renewcommand\headrule{}
% \fancypagestyle{plain}{
% 	\fancyhf{}% Clear header/footer
%   	%\fancyhead[C]{WILDMOD - Standard EF}  	
%   	\fancyhead[L]{Advanced Topic in Mathematical Logic}
%   	\fancyhead[R]{Christian d'Elbée}
% 	\cfoot{Page \thepage \ of \pageref{LastPage}}
% }
\pagestyle{plain}% Set page style to plain




% Show the labels
%\usepackage{showlabels}



% Theorems

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{observation}[theorem]{Observation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem*{theorem*}{Theorem}
\newtheorem{example}[theorem]{Example}



\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{exercise}{Exercise}
\newtheorem{claim}{Claim}
\newtheorem*{notation}{Notation}
\newtheorem*{problem}{\textbf{Problem}}










% General math


% Mathbb:
\newcommand\R{\mathbb{R}}	
\newcommand\C{\mathbb{C}}
\newcommand\Q{\mathbb{Q}}
\newcommand\N{\mathbb{N}}
\newcommand\Z{\mathbb{Z}}
\newcommand\F{\mathbb{F}}
\newcommand\HH{\mathbb{H}}
\newcommand\G{\mathbb{G}}
\newcommand\K{\mathbb{K}}
\newcommand\A{\mathbb{A}}
\newcommand\MM{\mathbb{M}}


% Mathcal:
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cK{\mathcal{K}}
\def\cP{\mathcal{P}}
\def\cG{\mathcal{G}}
\def\cL{\mathcal{L}}
\def\cX{\mathcal{X}}
\def\cQ{\mathcal{Q}}
\def\cH{\mathcal{H}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cF{\mathcal{F}}
\def\cU{\mathcal{U}}
\def\cZ{\mathcal{Z}}
\def\bM{\mathbb{M}}
\def\indd{\textnormal{ind}}
\def\Fac{\textnormal{Fac}}
\def\Vect{\mathrm{Vect}}
\def\Th{\operatorname{Th}}
\def\lcm{\operatorname{lcm}}




% Mathfrak:
\newcommand\p{\mathfrak{p}}
\newcommand\q{\mathfrak{q}}
\newcommand\rr{\mathfrak{r}}
\newcommand\Spec{\mathrm{Spec}}
\newcommand\m{\mathfrak{m}}
\newcommand\fS{\mathfrak{S}}



% Mathscr: 
\newcommand\scrA{\mathscr{A}}
\newcommand\GG{\mathscr{G}}
\newcommand\NN{\mathscr{N}}
\newcommand\CC{\mathscr{C}}
\newcommand\LL{\mathscr{L}}
\newcommand\LLf{\mathscr{L}_{\mathrm{fields}}}
\newcommand\LLr{\mathscr{L}_{\mathrm{ring}}}
\newcommand\LLm{\mathscr{L}_{\mathrm{m}}}



% Mathrm:
\newcommand{\ACFG}{\mathrm{ACFG}}
\newcommand{\ACF}{\mathrm{ACF}}
\newcommand{\ACFA}{\mathrm{ACFA}}
\newcommand{\ACFH}{\mathrm{ACFH}}
\newcommand{\NFCP}{\mathrm{NFCP}}
\newcommand{\RCF}{\mathrm{RCF}}
\newcommand{\PAC}{\mathrm{PAC}}
\newcommand{\PACG}{\mathrm{PACG}}
\newcommand{\Psf}{\mathrm{Psf}}
\newcommand{\DCF}{\mathrm{DCF}}
\newcommand{\SCF}{\mathrm{SCF}}
\newcommand{\ACVF}{\mathrm{ACVF}}
\newcommand{\acl}{\mathrm{acl}}
\newcommand{\dcl}{\mathrm{dcl}}
\newcommand{\cl}{\mathrm{cl}}
\newcommand{\Sg}{\mathrm{Sg}}
\newcommand{\End}{\mathrm{End}}
\newcommand{\Endd}{\mathrm{Endd}}
\newcommand{\di}{\mathrm{dim}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\expo}{\mathrm{exp}}
\newcommand{\dg}{\mathrm{deg}}
\newcommand{\Frob}{\mathrm{Frob}}
\newcommand{\Frac}{\mathrm{Frac}}
\newcommand{\Mat}{\mathrm{Mat}}
\newcommand{\alg}{\mathrm{alg}}
\newcommand{\Gal}{\mathrm{Gal}}
\newcommand{\chara}{\mathrm{char}}
\newcommand{\ac}{\mathrm{ac}}
\newcommand{\eq}{\mathrm{eq}}
\newcommand{\pw}{\mathrm{pw}}
\newcommand{\tp}{\mathrm{tp}}
\newcommand{\lstp}{\mathrm{lstp}}
\newcommand{\dv}{\mathrm{div}}
\newcommand{\RM}{\mathrm{RM}}
\newcommand{\DM}{\mathrm{DM}}  
\newcommand{\Proj}{\mathrm{Proj}} 
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\opp}{\mathrm{opp}}
\newcommand{\Graph}{\mathrm{Graph}}
\newcommand{\RG}{\mathrm{RG}}
\newcommand{\st}{\mathrm{st}}
\newcommand{\ld}{\mathrm{ld}}
\newcommand{\Sk}{\mathrm{Sk}}
\newcommand{\Av}{\mathrm{Av}}
\newcommand{\Circle}{\mathrm{Circle}}



% Operators/functions:
\def\seq{\subseteq}
\def\sneq{\subsetneq}
\newcommand{\set}[1]{\left\{ {#1} \right\}}
\newcommand{\vect}[1]{\langle {#1} \rangle}
\newcommand{\abs}[1]{\lvert {#1} \rvert}
\newcommand{\sv}[1]{\sqrt{ \vect{ {#1} } }}
\newcommand{\oF}[1]{\F^\alg_{{#1}}}
  
\newcommand{\brac}[2]{\left[ {#1} , {#2} \right]}

\newcommand{\Tds}[1]{T_{#1}^{2-\mathrm{sort}}} 


\newcommand{\ol}[1]{\overline{#1}}  

\DeclareMathOperator{\fix}{fix}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Soc}{Soc}
\DeclareMathOperator{\Hol}{Hol}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\Grp}{Grp}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\Jac}{Jac}
\DeclareMathOperator{\trdeg}{Trdeg}
\DeclareMathOperator{\EM}{EM}
\DeclareMathOperator{\cf}{cf}




\newcommand\abplus{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily ab}}}{\oplus}}}

\newcommand{\kappabar}{\bar{\kappa}}

% Colors:
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\newcommand{\afb}[1]{\textcolor{airforceblue}{#1}}
  
  
  
  
  


%Adler's (modified) code for independence relation

\def\IND{\setbox0=\hbox{$x$}\kern\wd0\hbox to 0pt{\hss$\mid$\hss}
\lower.9\ht0\hbox to 0pt{\hss$\smile$\hss}\kern\wd0}
\def\NotIND{\setbox0=\hbox{$x$}\kern\wd0\hbox to 0pt{\mathchardef\nn=12854\hss$\nn$\kern1.4\wd0\hss}\hbox to 0pt{\hss$\mid$\hss}\lower.9\ht0 \hbox to 0pt{\hss$\smile$\hss}\kern\wd0}


\def\ind{\mathop{\mathpalette\IND{}}}
\def\nind{\mathop{\mathpalette\NotIND{}}}




\def\indi#1{\mathop{\mathpalette\IND{}^{\!\!\!\!\rlap{$\scriptstyle{#1}$}\,\,\,\,}}}

\def\nindi#1{\mathop{\mathpalette\NotIND{}^{\!\!\!\rlap{$\scriptstyle{#1}$}\,\,\,}}}








% Setword Function
\makeatletter
\newcommand{\setword}[2]{%
  \phantomsection
  #1\def\@currentlabel{\unexpanded{#1}}\label{#2}%
}
\makeatother


%Solving the "Models" problem:
\renewcommand{\models}{\vDash}


%More shortcuts


\renewcommand\labelitemi{$\centerdot$}



% \usepackage[
% backend=biber,doi=false,url=false,isbn=false
% ,eprint=false,maxnames=3]{biblatex}
% \addbibresource{biblio.bib}




